ProbeAct: Probe-Guided Training-Free Failure Recovery in Vision-Language-Action Models

Vision-Language-Action (VLA) models demonstrate strong perfor-1 mance on language-conditioned robotic manipulation within their training dis-2 tribution, yet their generalization capabilities remain fundamentally limited. They3 lack the robustness required to handle perturbations, frequently failing when con-4 fronted with lighting changes, altered camera viewpoints, or small initial-state5 variations. We propose PROBEACT, a training-free runtime intervention frame-6 work that detects and recovers from grasping and placement failures in pre-7 trained VLA policies without modifying their weights or requiring additional8 demonstrations. PROBEACT combines three components: (i) a lightweight multi-9 target hidden-state probe that predicts the 3D positions of task-relevant objects10 from intermediate VLA features, with Hungarian-matched identity tracking for11 multi-object scenes; (ii) an object-agnostic kinematic state machine that detects12 grasp, transport, and placement failures using only gripper-internal signals and13 end-effector kinematics; and (iii) a hierarchical Control Barrier Function (CBF)14 filter that encodes repeated-failure locations as soft safe-set constraints, mini-15 mally correcting VLA actions while preserving baseline behavior. As a plug-and-16 play, training-free intervention loop, PROBEACT is orthogonal to existing train-17 ing pipelines. Evaluated on the LIBERO-plus benchmark, our framework acts as18 a universal safety net, improving the success rate of the OpenVLA-OFT model19 from 69.6% to 74.1%, while demonstrating broad applicability to both base and20 fine-tuned VLA policies.

==> table/ablation_probe.tex <==
\begin{table}[t]
\centering
\caption{Layer $\times$ Pooling Comparison (Recovery Direction $R^2$)}
\label{tab:layer_pooling}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Layer} & 
\textbf{img spatial} &
\textbf{img mean} & \textbf{last} & \textbf{lang mean} \\
\hline
8  & \textbf{0.968} & 0.926 & 0.815 & 0.869 \\
12 & 0.958 & 0.919 & 0.856 & 0.879 \\
16 & 0.947& 0.919 & 0.877 & 0.894 \\
20 & 0.947 & 0.918 & 0.886 & 0.921 \\
24 & 0.934 & 0.912 & 0.875 & 0.910 \\
28 & 0.934 & 0.912 & 0.861 & 0.914 \\
\hline
\end{tabular}

\vspace{0.4em}
\footnotesize{$\star$ Layer 8 (shallow) outperforms deeper layers --- spatial information is encoded early.}
\end{table}

==> table/main_results.tex <==
\begin{table}[tbp]
\centering
\caption{Comparison of success rates across LIBERO-plus categories (\%).}
\label{tab:performance_comparison}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
Model & Camera & Robot & Language & Light & Background & Noise & Layout & Total \\
\midrule
OpenVLA        & 0.8  & 3.5  & 23.0 & 8.1  & 34.8 & 15.2 & 28.5 & 15.6 \\
NORA           & 2.2  & 37.0 & 65.1 & 45.7 & 58.6 & 12.8 & 62.1 & 39.0 \\
WorldVLA       & 0.1  & 27.9 & 41.6 & 43.7 & 17.1 & 10.9 & 38.0 & 25.0 \\
UniVLA         & 1.8  & 46.2 & 69.6 & 69.0 & 81.0 & 21.2 & 31.9 & 43.9 \\
$\pi_0$        & 13.8 & 6.0  & 58.8 & 85.0 & 81.4 & 79.0 & 68.9 & 53.6 \\
$\pi_0$-Fast   & 65.1 & 21.6 & 61.0 & 73.2 & 73.2 & 74.4 & 68.8 & 61.6 \\
RIPT-VLA       & 55.2 & 31.2 & 77.6 & 88.4 & 91.6 & 73.5 & 74.2 & 68.4 \\
\midrule
OpenVLA-OFT    & 56.4 & 31.9 & 79.5 & 88.7 & 93.3 & 75.8 & 74.2 & 69.6 \\
\textbf{\method} (\textit{ours}) & \textbf{63.8} & \textbf{40.3} & \textbf{82.0} & \textbf{93.6} & \textbf{93.5} & \textbf{76.8} & \textbf{80.9} & \textbf{74.1} \\
\textit{Improvement} ($\Delta$) & \textit{+7.4} & \textit{+8.4} & \textit{+2.5} & \textit{+4.9} & \textit{+0.2} & \textit{+1.0} & \textit{+6.7} & \textit{+4.5} \\
\bottomrule
\end{tabular}
}
\end{table}
